Multi-Sample Online Learning for Probabilistic Spiking Neural Networks

Spiking Neural Networks (SNNs) capture some of the efficiency of biological brains for inference and learning via the dynamic, online, event-driven processing of binary time series. Most existing learning algorithms for SNNs are based on deterministic neuronal models, such as leaky integrate-and-fire, and rely on heuristic approximations of backpropagation through time that enforce constraints such as locality. In contrast, probabilistic SNN models can be trained directly via principled online, local, update rules that have proven to be particularly effective for resource-constrained systems. This paper investigates another advantage of probabilistic SNNs, namely their capacity to generate independent outputs when queried over the same input. It is shown that the multiple generated output samples can be used during inference to robustify decisions and to quantify uncertainty -- a feature that deterministic SNN models cannot provide. Furthermore, they can be leveraged for training in order to obtain more accurate statistical estimates of the log-loss training criterion, as well as of its gradient. Specifically, this paper introduces an online learning rule based on generalized expectation-maximization (GEM) that follows a three-factor form with global learning signals and is referred to as GEM-SNN. Experimental results on structured output memorization and classification on a standard neuromorphic data set demonstrate significant improvements in terms of log-likelihood, accuracy, and calibration when increasing the number of samples used for inference and training.

==> experiments-comp.tex <==
\section{Experimental Comparison} \label{sec:experiments-comp}

\vspace{3cm}


==> importance_weighted.tex <==
\section{Importance-Weighted Multi-Sample Online Learning for SNNs}




\begin{comment}
In order to obtain an online rule, we aim at minimizing at each time $t$ the discounted version of the upper bound $\set{L}_{\bmx_{\leq T}}^K(\bmtheta)$ in \eqref{eq:iw-elbo-T} given as
\begin{align} \label{eq:iw-elbo}
    \set{L}_{\bmx_{\leq t}}^{K,\gamma}(\bmtheta) := - \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq t}^{1:K}||\bmx_{\leq t})}\Big[ \log R_{\bmtheta^\text{X},t}^{K,\gamma}\Big] = 
    - \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq t}^{1:K}||\bmx_{\leq t})}\Big[ \log \frac{1}{K} \sum_{k=1}^K \exp\Big( v_{\bmtheta^\text{X},t}^{k,\gamma} \Big) \Big],
    %- \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq t}^{1:K}||\bmx_{\leq t})}\Big[ \log \underbrace{ \frac{1}{K} \sum_{k=1}^K \exp\Big( v_{\bmtheta^\text{X},t}^{k,\gamma} \Big)}_{:=~ R_{\bmtheta^\text{X},t}^{K,\gamma}}  \Big],
\end{align}
where a discount factor $\gamma \in (0,1)$ is introduced to address the batch processing required in $R_{\bmtheta^\text{X},T}^K$. The discounted version of the importance-weighted estimator $R_{\bmtheta^\text{X},t}^{K,\gamma}$ can be obtained by using the discounted values $v_{\bmtheta^\text{X},t}^{k,\gamma}$ in \eqref{eq:gem-log-weight}. 
\end{comment}




The {\MBVLSNN} rule introduced above leverages the $K$ compartments to improve the MC estimate of the gradient $\grad_{\bmtheta} L_{\bmx_{\leq T}}(\bmtheta)$ of the lower bound \eqref{eq:single-elbo-batch} of the log-likelihood $\log p_{\bmtheta}(\bmx_{\leq T})$. In this section, we consider an alternative approach that uses multiple compartments to obtain an increasingly more accurate bound on the log-likelihood. The approach follows the principles of the importance weighting method introduced in \cite{mnih2016variational, burda2015importance, domke2018iwvi} for conventional probabilistic models. 


\begin{comment}
\subsection{{\IWVLSNN}: Importance-Weighted VLSNN}

In this section, we develop an online local learning rule that maximizes the importance-weighted lower bound $L_{\bmx_{\leq t}}^K(\bmtheta)$ in \eqref{eq:multi-elbo}. We refer to the rule as Importance-Weighted Variational online Learning for SNNs ({\IWVLSNN}). {\IWVLSNN} updates the model parameters $\bmtheta$ via SGD in the direction of the gradient $\grad_{\bmtheta} L_{\bmx_{\leq t}}^K(\bmtheta)$, which is obtained using REINFORCE as
\begin{align} \label{eq:multi-elbo-grad}
    \grad_{\bmtheta}& L_{\bmx_{\leq t}}^K(\bmtheta) = \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq t}^{1:K} || \bmx_{\leq t-1})} \bigg[ \cr
    &\sum_{k=1}^K \tilde{v}_{\bmtheta^\text{X},t}^k \cdot \sum_{t'=0}^{t-1} \gamma^{t'} \sum_{i \in \set{X}} \grad_{\bmtheta} \bar{H}\big( x_{i,t-t'}, \sigma(u_{i,t-t'}^k) \big) \cr 
    &+ \ell_{\bmtheta^\text{X},t} \cdot \sum_{k=1}^K \sum_{t'=1}^t \sum_{i \in \set{H}} \grad_{\bmtheta} \bar{H} \big( h_{i,t'}^k, \sigma(u_{i,t'}^k) \big) \bigg].
\end{align}
In \eqref{eq:multi-elbo-grad}, we have defined $\bmv_{\bmtheta^\text{X},t} = (v_{\bmtheta^\text{X},t}^1, \ldots, v_{\bmtheta^\text{X},t}^K)$ as the vector of unnormalized log-weights of the samples at time $t$ in \eqref{eq:multi-elbo} using temporal average operator as
\begin{subequations} \label{eq:iw-quantities}
\begin{align} \label{eq:unnorm-weights-online}
    v_{\bmtheta^\text{X},t}^k = \big\langle w_{\bmtheta^\text{X},t}^k \big\rangle_\gamma = \big\langle \sum_{i \in \set{X}} \bar{H}\big( x_{i,t}, \sigma(u_{i,t}^k) \big) \big\rangle_\gamma,
\end{align}
and the normalized weights $\tilde{\bmv}_{\bmtheta^\text{X},t} = (\tilde{v}_{\bmtheta^\text{X},t}^1, \ldots, \tilde{v}_{\bmtheta^\text{X},t}^K)$ are defined using the SoftMax function over $K$ samples as
\begin{align} \label{eq:norm-weights-online}
    \tilde{\bmv}_{\bmtheta^\text{X},t} = \text{SoftMax} \big( \bmv_{\bmtheta^\text{X},t} \big), %~~\text{where}~~ \tilde{v}_{\bmtheta^\text{X},t}^k = \text{SoftMax}^k \big( \bmv_{\bmtheta^\text{X},t} \big) = \frac{ \exp\big( v_{\bmtheta^\text{X},t}^k \big)}{\sum_{k'=1}^K \exp\big( v_{\bmtheta^\text{X},t}^{k'} \big) }.
\end{align}
where 
\begin{align*}
    \tilde{v}_{\bmtheta^\text{X},t}^k = \text{SoftMax}^k \big( \bmv_{\bmtheta^\text{X},t} \big) = \frac{ \exp\big( v_{\bmtheta^\text{X},t}^k \big)}{\sum_{k'=1}^K \exp\big( v_{\bmtheta^\text{X},t}^{k'} \big) }.
\end{align*}
The learning signal $\ell_{\bmtheta^\text{X},t}$ at time $t$ in \eqref{eq:multi-elbo} can be expressed using the LogSumExp function as 
\begin{align} \label{eq:iw-ls-online}
    \ell_{\bmtheta^\text{X},t} = \text{LogSumExp}\big( \bmv_{\bmtheta^\text{X},t} \big) - \log K, %~~\text{where}~~ \text{LogSumExp}\big( \bmv_{\bmtheta^\text{X},t} \big) = \log \sum_{k=1}^K \exp\big( v_{\bmtheta^\text{X},t}^k \big).
\end{align}
where
\begin{align*}
    \text{LogSumExp}\big( \bmv_{\bmtheta^\text{X},t} \big) = \log \sum_{k=1}^K \exp\big( v_{\bmtheta^\text{X},t}^k \big).
\end{align*}
\end{subequations}
The resulting learning algorithm {\IWVLSNN} based on the MC estimate of the gradient \eqref{eq:multi-elbo-grad} operates as follows. 

In a $K$-compartment SNN, at each time $t=1,2,\ldots,$ all compartments within visible neurons are clamped to the data $\bmx_{\leq t}$, while each hidden neuron $i \in \set{H}$ emits a spike $h_{i,t}^k = 1$ with probability $\sigma(u_{i,t}^k)$ at each compartment $k=1,\ldots,K$. Then, the model parameters are updated as follows. As illustrated in Fig.~\ref{fig:model-learning}, the CP collects the binary negative cross-entropy values $\{ \bar{H}\big( x_{i,t}, \sigma(u_{i,t}^k) \big) \}_{k=1}^K$ of all compartments from all visible neurons $i \in \set{X}$. These are used by the CP to compute the importance weights $\bmv_{\bmtheta^\text{X},t}$ from \eqref{eq:unnorm-weights-online}; the normalized importance weights $\tilde{\bmv}_{\bmtheta^\text{X},t}$ in \eqref{eq:norm-weights-online}; and the learning signal $\ell_{\bmtheta^\text{X},t}$ from \eqref{eq:iw-ls-online}. Finally, the normalized weights $\{\tilde{v}_{\bmtheta^\text{X},t}^k\}_{k=1}^K$ are fed back from the CP to all visible neurons $\set{X}$, while a common learning signal $\ell_{\bmtheta^\text{X},t}$ is fed back to all hidden neurons $\set{H}$. Finally, for each neuron $i$, {\IWVLSNN} updates the local model parameters $\bmtheta_i$ as 
\begin{subequations} \label{eq:iw-update}
\begin{align}
    & \Delta \vartheta_i =
    \begin{cases}
        \sum_{k=1}^K \tilde{v}_{\bmtheta^\text{X},t}^k \cdot \big\langle x_{i,t} - \sigma(u_{i,t}^k) \big\rangle_\gamma, ~\text{if}~ i \in \set{X} \\
        \big( \ell_{\bmtheta^\text{X},t} - b_{t}^{\vartheta_i} \big) \cdot \sum_{k=1}^K \big\langle h_{i,t}^k - \sigma(u_{i,t}^k) \big\rangle_\kappa, ~\text{if}~ i \in \set{H}
    \end{cases} \label{eq:iw-update-bias} \\
    & \Delta w_{j,i} =
    \begin{cases}
        \sum_{k=1}^K \tilde{v}_{\bmtheta^\text{X},t}^k \cdot \big\langle \big( x_{i,t} - \sigma(u_{i,t}^k) \big) \cdot \overra{s}_{j,t-1}^{k} \big\rangle_\gamma, \\%~~\text{if}~~ i \in \set{X} \\
        \big( \ell_{\bmtheta^\text{X},t} - b_{t}^{w_{j,i}} \big) \cdot \sum_{k=1}^K \Big\langle \big( h_{i,t}^k - \sigma(u_{i,t}^k) \big) \cdot \overra{s}_{j,t-1}^{k} \big\rangle_\kappa, %~~\text{if}~~ i \in \set{H}
        \end{cases} \label{eq:iw-update-synaptic} \\
    & \Delta w_i =
    \begin{cases}
        \sum_{k=1}^K \tilde{v}_{\bmtheta^\text{X},t}^k \cdot \big\langle \big( x_{i,t} - \sigma(u_{i,t}^k) \big) \cdot \overla{x}_{i,t-1} \big\rangle_\gamma, \\%~~\text{if}~~ i \in \set{X} \\
        \big( \ell_{\bmtheta^\text{X},t} - b_{t}^{w_i} \big) \cdot \sum_{k=1}^K \big\langle \big( h_{i,t}^k - \sigma(u_{i,t}^k) \big) \cdot \overla{h}_{i,t-1}^k \big\rangle_\kappa, %~~\text{if}~~ i \in \set{H}
    \end{cases} \label{eq:iw-update-feedback}
\end{align}
\end{subequations}
with constants $\gamma, \kappa \in (0,1)$. For each hidden neuron $i \in \set{H}$, the baseline $\bmb_{i,t}$ can be introduced to minimize the variance of the gradient estimator \eqref{eq:multi-elbo-grad} as \cite{peters2008reinforcement}
\begin{align} \label{eq:iw-baseline}
    \bmb_{i,t} = \frac{ \big\langle \ell_{\bmtheta^\text{X},t} \cdot \sum_{k=1}^K \big( \bme_{i,t}^k \big)^2 \big\rangle_{\kappa_b} }{\big\langle \sum_{k=1}^K \big( \bme_{i,t}^k \big)^2 \big\rangle_{\kappa_b}}.
\end{align}
for some constant $\kappa_b \in (0,1)$.

\end{comment}

\iffalse
\begin{align*}
    \Delta \bmtheta_i = \eta \cdot 
    \begin{cases}
        \sum_{k=1}^K \tilde{v}_{\bmtheta^\text{X},t}^k \cdot \big\langle \grad_{\bmtheta_i} \bar{H}\big( x_{i,t}, \sigma(u_{i,t}^k) \big) \big\rangle, ~~\text{if}~~ i \in \set{X} \\
        \big( \ell_{\bmtheta^\text{X},t} - \bmb_{i,t} \big) \cdot \sum_{k=1}^K \big\langle \grad_{\bmtheta_i} \bar{H} \big( h_{i,t}^k, \sigma(u_{i,t}^k) \big) \big\rangle, ~~\text{if}~~ i \in \set{H}
    \end{cases}
\end{align*}
\fi


\subsection{Interpreting {\IWVLSNN}}

The update rule \eqref{eq:iw-update} follows the three-factor format in \eqref{eq:three-factor}. The dependence on the post-synaptic error, post-synaptic feedback trace, and pre-synaptic synaptic trace is applied for each compartment as for {\VLSNN} and {\MBVLSNN}, while the learning signal is given in different form to each neuron. For visible neurons, the normalized importance weights $\{ \tilde{v}_{\bmtheta^\text{X},t}^k \}_{k=1}^K$ are given as learning signals, with the contribution of each compartment being weighted by $\tilde{v}_{\bmtheta^\text{X},t}^k$. From \eqref{eq:norm-weights-online}, the normalized weight $\tilde{v}_{\bmtheta^\text{X},t}^k$ measures the relative effectiveness of the random realizations of the hidden neurons within the $k$th compartment in reproducing the desired behavior of the visible neurons. In contrast, for the hidden neurons, the learning signal $\ell_{\bmtheta^\text{X},t}$ in \eqref{eq:iw-ls-online} is given as a global feedback, indicating how effective their current overall behavior across all compartments is in ensuring the maximization of the likelihood of observation $\bmx_{\leq t}$. Note that this signal is shared across all compartments.

\vspace{-0.1cm}
\subsection{Communication Load}

% \begin{table}[t]
% \caption{Learning Communication Loads (in real numbers)}
% \label{tab:comparison}
% \vspace{-0.4cm}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Scheme & Unicast $\CNtoCP$ & Broadcast $\CCPtoN$\\
% \midrule
% {\VLSNN} & $\CNtoCP^{(K=1)} = |\set{X}|$ & $\CCPtoN^{(K=1)} = |\set{H}|$ \\
% {\MBVLSNN} & $K|\set{X}|$ & $K|\set{H}|$ \\
% {\IWVLSNN} & $K|\set{X}|$ & $K|\set{X}| + |\set{H}|$ \\
% {\IWbVLSNN} & $K|\set{X}|$ & $K(|\set{X}| + |\set{H}|)$ \\
% {\GEMVLSNN} & $K|\set{X}|$ & $K(|\set{X}| + |\set{H}|)$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vspace{-0.5cm}
% \end{table}

From the description of {\IWVLSNN} given above, as illustrated in Fig.~\ref{fig:model-learning}, the unicast communication load of {\IWVLSNN} from neuron to CP is $\CNtoCP = K \CNtoCP^{(K=1)} = K|\set{X}|$ real numbers; while the broadcast communication load from CP to neurons is $\CCPtoN = K |\set{X}| + |\set{H}|$. As compared to {\MBVLSNN} whose broadcast load is $K |\set{H}|$, the broadcast communication load of {\IWVLSNN} can be smaller if the number of hidden neurons is large.

%includes $K |\set{X}|$ normalized weights of the compartments to visible neurons and $|\set{H}|$ common learning signals given to hidden neurons. 

\iffalse    
As investigated in \cite{domke2018iwvi}, maximizing the bound $L_{\bmx_{\leq T}}^K(\bmtheta)$ minimizes the KL divergence between the self-normalized importance sampling (NIS) distribution over a batch of $K$ samples, i.e., obtained from the SoftMax function, and the true posterior. After learning, for inference at each time $t$, the expectation over the true posterior can be approximated as 
%    \begin{align} \label{eq:multi-vi}
%        \mathbb{E}_{p_{\bmtheta}(\bmh_{\leq T} | \bmx_{\leq T})} \big[ f(\bmh_{\leq T}) \big] &\approx \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq T}^{1:K} || \bmx_{\leq T-1})} \Big[ \frac{\sum_{k=1}^K \exp \big( w_{\bmtheta^\text{X}}^k \big) \cdot f(\bmh_{\leq T}^k) }{ \sum_{k'=1}^K \exp \big( w_{\bmtheta^\text{X}}^{k'} \big) } \Big] \cr 
%        &= \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq T}^{1:K} || \bmx_{\leq T-1})} \Big[ \sum_{k=1}^K \tilde{w}_{\bmtheta^\text{X}}^k \cdot f(\bmh_{\leq T}^k) \Big],
%    \end{align}
\begin{align} \label{eq:multi-vi}
    \mathbb{E}_{p_{\bmtheta}(\bmh_{\leq t}| \bmx_{\leq t})} \big[ f(\bmh_{\leq t})\big] &\approx \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq t}^{1:K} || \bmx_{\leq t-1})} \bigg[ \sum_{k=1}^K \text{SoftMax}^k\Big( \sum_{t'=1}^t \bmw_{\bmtheta^\text{X},t'} \Big) \cdot f(\bmh_{\leq t}^k) \bigg]
\end{align}
where the normalized log-weights at time $t$ are computed using the SoftMax function, without temporal average operator.
\fi


\begin{comment}

\subsection{{\IWVLSNN} with Per-Compartment Learning Signal} 

As per \eqref{eq:iw-update}, {\IWVLSNN} applies the same baseline \eqref{eq:iw-baseline} to all compartments of the hidden neurons. Hence, unlike the differentiated per-compartment feedback signals sent to the visible neurons, {\IWVLSNN} does not implement relative credit assignment across the $K$ compartments for hidden neurons. The common learning signal applied to each compartment may not be sufficiently specific and, as a result, it may suffer from high variance. In order to address this issue, we introduce per-compartment learning signals denoted by $\ell_{\bmtheta^\text{X},t}^k$ for all compartments $k=1,\ldots,K$ of the hidden neurons. Following \cite{mnih2016variational}, a per-compartment learning signal can be defined by subtracting a term dependent on the contribution of the other compartments to the learning signal in \eqref{eq:multi-elbo} as
\begin{align*}
    \ell_{\bmtheta^\text{X},t}^k = \ell_{\bmtheta^\text{X},t} - \log \frac{1}{K} \Big(& \sum_{k' \neq k} \exp\Big( v_{\bmtheta^\text{X},t}^{k'} \Big) + \exp\Big( \frac{\sum_{k' \neq k} v_{\bmtheta^\text{X},t}^{k'}}{K-1} \Big)  \Big).
\end{align*}

With this approach, the CP needs to compute the per-compartment learning signals $\{\ell_{\bmtheta^\text{X},t}^k\}_{k=1}^K$ with information collected from the visible neurons $\set{X}$, which are then fed back to all hidden neurons $\set{H}$. Instead of the update rule \eqref{eq:iw-update}, this alternative rule, referred to as {\IWbVLSNN}, updates the local model parameters $\bmtheta_i$ of each neuron $i$ as
\begin{align} \label{iw-update-b}
    \Delta \bmtheta_i =
    \begin{cases}
        \sum_{k=1}^K \tilde{v}_{\bmtheta^\text{X},t}^k \cdot \big\langle \grad_{\bmtheta_i} \bar{H}\big( x_{i,t}, \sigma(u_{i,t}^k)\big) \big\rangle_\gamma, ~\text{if}~ i \in \set{X} \\
        \sum_{k=1}^K \ell_{\bmtheta^\text{X},t}^k \cdot \big\langle \grad_{\bmtheta_i} \bar{H}\big( h_{i,t}^k, \sigma(u_{i,t}^k) \big) \big\rangle_\kappa, ~\text{if}~ i \in \set{H}.
    \end{cases}
\end{align}
As a result, as illustrated in Fig.~\ref{fig:model-learning}, the broadcast communication load from CP to neurons includes the normalized weights of the compartments $\{ \tilde{v}_{\bmtheta^\text{X},t}^k \}_{k=1}^K$ to visible neurons and $\{ \ell_{\bmtheta^\text{X},t}^k \}_{k=1}^K$ per-compartment learning signals to hidden neurons, entailing the load $\CCPtoN = K(|\set{X}|+|\set{H}|)$.

\end{comment}







==> minibatch.tex <==
\section{Mini-Batch VLSNN}



It is anticipated that using a mini-batch of $K$ samples can reduce the variance of the single-sample estimator. 

\vspace{2cm}


\begin{comment}
\subsection{{\VLSNN}: Variational Online Learning for SNNs}

In online learning, the model parameters $\bmtheta$ are updated at each time $t$ based on the data $\bmx_{\leq t}$ observed so far. To this end, at each time $t=1,2,\ldots$, the visible neurons are clamped to the data $\bmx_t$, and each hidden neuron $i \in \set{H}$ emits a spike $h_{i,t} = 1$ with probability $\sigma(u_{i,t})$ from \eqref{eq:spike-prob-ind}. Weights updates are carried out using a three-factor rule of the form \eqref{eq:three-factor} as follows. A central processor (CP) collects the binary negative cross-entropy values $\bar{H}\big( x_{i,t}, \sigma(u_{i,t}) \big)$ in \eqref{eq:log-prob-ind} from all visible neurons $i \in \set{X}$, and it computes the learning signal
\begin{align} \label{eq:single-ls}
    \ell_{\bmtheta^\text{X},t} = \Big\langle \sum_{i \in \set{X}} \bar{H}\big( x_{i,t}, \sigma(u_{i,t}) \big) \Big\rangle_\gamma,
\end{align}
for some constant $\gamma \in (0,1)$. The learning signal is then fed back from the CP to all hidden neurons $\set{H}$. Finally, each neuron $i$ updates the local model parameters $\bmtheta_i$ as $\bmtheta_i \leftarrow \bmtheta_i + \eta \cdot \Delta \bmtheta_i$ with a learning rate $\eta$, where each component of $\Delta \bmtheta_i$ is given as
\begin{subequations} \label{eq:single-update}
\begin{align} 
    &\Delta \vartheta_i =
    \begin{cases}
        \big\langle x_{i,t} - \sigma(u_{i,t}) \big\rangle_\gamma, ~\text{if}~ i \in \set{X} \\
            \big( \ell_{\bmtheta^\text{X},t} - b_{t}^{\vartheta_i} \big) \cdot \big\langle h_{i,t} - \sigma(u_{i,t}) \big\rangle_\kappa, ~\text{if}~ i \in \set{H}
    \end{cases} \label{eq:single-update-bias} \\
    &\Delta w_{j,i} =
    \begin{cases}
        \big\langle \big( x_{i,t} - \sigma(u_{i,t}) \big) \cdot \overra{s}_{j,t-1} \big\rangle_\gamma, \\%~~\text{if}~~ i \in \set{X} \\
            \big( \ell_{\bmtheta^\text{X},t} - b_{t}^{w_{j,i}} \big) \cdot \big\langle \big( h_{i,t} - \sigma(u_{i,t}) \big) \cdot \overra{s}_{j,t-1} \big\rangle_\kappa, %~~\text{if}~~ i \in \set{H}
    \end{cases} \label{eq:single-update-synaptic} \\
    &\Delta w_i =
    \begin{cases}
        \big\langle \big( x_{i,t} - \sigma(u_{i,t}) \big) \cdot \overla{x}_{i,t-1} \big\rangle_\gamma, \\% ~~\text{if}~~ i \in \set{X} \\
        \big( \ell_{\bmtheta^\text{X},t} - b_{t}^{w_i} \big) \cdot \big\langle \big( h_{i,t} - \sigma(u_{i,t}) \big) \cdot \overla{h}_{i,t-1} \big\rangle_\kappa, % ~~\text{if}~~ i \in \set{H}
    \end{cases} \label{eq:single-update-feedback}
\end{align}
\end{subequations}
with a constant $\kappa \in (0,1)$. The baselines $\bmb_{i,t} = \{ \{b_t^{w_{j,i}} \}_{j \in \set{P}_i}, b_t^{w_i}, b_t^{\vartheta_i} \}$ are control variates introduced as means to minimize the variance of the gradient estimator for hidden neuron $i \in \set{H}$. Following the approach in \cite{peters2008reinforcement}, the optimized baseline can be evaluated as 
\begin{align*}
    \bmb_{i,t} = \frac{ \big\langle \ell_{\bmtheta^\text{X},t} \cdot \bme_{i,t}^2  \big\rangle_{\kappa_b} }{ \big\langle \bme_{i,t}^2 \big\rangle_{\kappa_b} },
\end{align*}
for some constant $\kappa_b \in (0,1)$, with $\bme_{i,t} = \big\langle \grad_{\bmtheta_i} \bar{H}\big( h_{i,t}, \sigma(u_{i,t})\big) \big\rangle_\kappa$ denoting the {\em eligibility trace} of neuron $i$ at time $t$. We refer to the online rule \eqref{eq:single-update} as Variational online Learning for SNNs ({\VLSNN}).

\iffalse
\begin{align*}
    \Delta \bmtheta_i = \eta \cdot 
    \begin{cases}
        \big\langle \grad_{\bmtheta_i} \bar{H}\big( x_{i,t}, \sigma(u_{i,t}) \big) \big\rangle, ~~\text{if}~~ i \in \set{X} \\
        \big( \ell_{\bmtheta^\text{X},t} - \bmb_{i,t} \big) \cdot \big\langle \grad_{\bmtheta_i} \bar{H} \big( h_{i,t}, \sigma(u_{i,t}) \big) \big\rangle, ~~\text{if}~~ i \in \set{H}
    \end{cases}
\end{align*}
\fi

\vspace{-0.1cm}
\subsection{Derivation of {\VLSNN}}

In order to make the paper self-contained and to facilitate the derivation of multi-compartment learning schemes, we present here a brief derivation of {\VLSNN}. To address the ML problem \eqref{eq:ml} in an online manner, {\VLSNN} aims at maximizing at each time $t$ a discounted version of a lower bound $L_{\bmx_{\leq T}}(\bmtheta)$ on the log-likelihood $\log p_{\bmtheta}(\bmx_{\leq T})$ of the observation $\bmx_{\leq T}$. Using Jensen's inequality, the lower bound is obtained as
\begin{align} \label{eq:single-elbo-batch}
    &\log p_{\bmtheta}(\bmx_{\leq T}) = \log \sum_{\bmh_{\leq T}} p_{\bmtheta}(\bmx_{\leq T}, \bmh_{\leq T}) \cr
    &~~ \geq \mathbb{E}_{ \bmh_{\leq T} \sim p_{\bmtheta^\text{H}}(\bmh_{\leq T} || \bmx_{\leq T-1}) } \Big[ \sum_{t=1}^T \sum_{i \in \set{X}} \bar{H}\big( x_{i,t}, \sigma(u_{i,t}) \big) \Big] \cr 
    &~~ := L_{\bmx_{\leq T}}(\bmtheta),
\end{align}
where we have used the notation
\begin{align} 
    p_{\bmtheta^\text{H}}(\bmh_{\leq T} || \bmx_{\leq T-1}) &= \prod_{t=1}^T p_{\bmtheta}(\bmh_{t} | \bmx_{\leq t-1}, \bmh_{\leq t-1}) \cr 
    &=  \prod_{t=1}^T \prod_{i \in \set{H}} p_{\bmtheta_i}(h_{i,t} | u_{i,t})
\end{align}
to indicate the causally conditioned distribution of hidden neurons, signals given the visible neurons, signals \cite{kramer1998directed}. We note that we have the decomposition
\begin{align*}
p_{\bmtheta}(\bmx_{\leq T}, \bmh_{\leq T}) = p_{\bmtheta^\text{H}}(\bmh_{\leq T} || \bmx_{\leq T-1}) p_{\bmtheta^\text{X}}(\bmx_{\leq T} || \bmh_{\leq T-1}),    
\end{align*}
where the causally conditioned distribution of visible neuron given hidden neurons is similarly defined as $p_{\bmtheta^\text{X}}(\bmx_{\leq T} || \bmh_{\leq T-1}) = \prod_{t=1}^T \prod_{i \in \set{X}} p_{\bmtheta_i}(x_{i,t}|u_{i,t})$ \cite{kramer1998directed}. We denote as $\bmtheta^\text{X} = \{ \bmtheta_i \}_{i \in \set{X}}$ and $\bmtheta^\text{H} = \{ \bmtheta_i \}_{i \in \set{H}}$ the collection of model parameters for visible $\set{X}$ and hidden $\set{H}$ neurons, respectively. Finally, we define the time-discounted version of the lower bound $L_{\bmx_{\leq T}}(\bmtheta)$ in \eqref{eq:single-elbo-batch} at time $t$ as 
\begin{align} \label{eq:single-elbo}
    L_{\bmx_{\leq t}}(\bmtheta) &= \mathbb{E}_{p_{\bmtheta^\text{H}}(\bmh_{\leq t} || \bmx_{\leq t-1})} \Big[ \cr 
    &~~ \underbrace{ \sum_{t'=0}^{t-1} \gamma^{t'} \sum_{i \in \set{X}} \bar{H}\big( x_{i,t-t'}, \sigma(u_{i,t-t'}) \big) }_{:=~ \ell_{\bmtheta^\text{X},t} } \Big],
\end{align}
where $0 < \gamma < 1$ is a discount factor.

The online local update rule {\VLSNN} in \eqref{eq:single-update} can be obtained by maximizing the lower bound $L_{\bmx_{\leq t}}(\bmtheta)$ in \eqref{eq:single-elbo} via SGD in the direction of a stochastic estimate of the gradient $\grad_{\bmtheta} L_{\bmx_{\leq t}}(\bmtheta)$. The gradient of \eqref{eq:single-elbo} is obtained from the standard REINFORCE gradient, which is estimated by drawing a single spiking signal $\bmh_{\leq t} \sim p_{\bmtheta^\text{H}}(\bmh_{\leq t} || \bmx_{\leq t-1})$ for the hidden neurons from the causally conditioned distribution \eqref{eq:causally-cond}. Note that, as explained in Sec.~\ref{sec:intro}, the limitation of a single sample is dictated by the presence of single-compartment neurons, i.e., $K = 1$. The resulting MC estimate of the gradient can be computed as \cite{jang19:spm}
\begin{eqnarray} \label{eq:single-elbo-grad}
    &&\grad_{\bmtheta} L_{\bmx_{\leq t}}(\bmtheta) = \sum_{t'=0}^{t-1} \gamma^{t'} \sum_{i \in \set{X}} \grad_{\bmtheta} \bar{H}\big( x_{i,t-t'}, \sigma(u_{i,t-t'})\big) \cr
    &&\quad \qquad+ \ell_{\bmtheta^\text{X},t} \cdot \sum_{t'=1}^t \sum_{i \in \set{H}} \grad_{\bmtheta} \bar{H}\big( h_{i,t'}, \sigma(u_{i,t'}) \big),
\end{eqnarray}
which yields the SGD-based learning rule as $\bmtheta \leftarrow \bmtheta + \eta \cdot \grad_{\bmtheta} L_{\bmx_{\leq t}}(\bmtheta)$ with a learning rate $\eta$. This can be seen to coincide with \eqref{eq:single-update} \cite{brea2013matching, jimenez2014stochastic, jang19:spm}.
\end{comment}

\subsection{Interpreting {\VLSNN}}

Following the discussion around \eqref{eq:three-factor}, the update rule \eqref{eq:single-update} has the form of a three-factor rule \cite{fremaux2016neuromodulated} and is local, with the exception of the learning signal $\ell_{\bmtheta^\text{X},t}$ used for the update of hidden neurons' parameters. For each neuron $i$, the gradients $\grad_{\bmtheta_i} L_{\bmx_{\leq t}}(\bmtheta)$ with respect to the local model parameters $\bmtheta_i$ from \eqref{eq:single-elbo-grad} contain three types of terms, namely the post-synaptic error $s_{i,t} - \sigma(u_{i,t})$ and post-synaptic feedback trace $\overla{s}_{i,t-1}$; pre-synaptic synaptic trace $\overra{s}_{j,t-1}$; and the common global learning signal $\ell_{\bmtheta^\text{X},t}$ in \eqref{eq:single-ls}. For hidden neurons $\set{H}$, the learning signal is used to guide the update, while the visible neurons $\set{X}$ do not use the learning signal. The common learning signal term $\ell_{\bmtheta^\text{X},t}$ in \eqref{eq:single-ls} can then be interpreted as indicating indicates how effective the current, randomly sampled, behavior of hidden neurons $\bmh_{\leq t}$ is in ensuring the maximization of the likelihood of the desired observation $\bmx_{\leq t}$ for the visible neurons. 

\vspace{-0.1cm}
\subsection{Communication Load}

As discussed, {\VLSNN} requires bi-directional communication. As seen in Fig.~\ref{fig:model-learning}, at each step $t$, first, unicast communication from visible neurons to CP is required in order to compute the learning signal $\ell_{\bmtheta^\text{X},t}$ by collecting information $\{ \bar{H}\big( x_{i,t}, \sigma(u_{i,t}) \big)\}_{i \in \set{X}}$ from all visible neurons. The resulting unicast communication load, from neurons to CP, is $\CNtoCP^{(K=1)} = |\set{X}|$ real numbers. The learning signal is then sent back to all hidden neurons, resulting a broadcast communication load from CP to neurons equal to $\CCPtoN^{(K=1)} = |\set{H}|$ real numbers.




As discussed, {\VLSNN} is based on a MC estimate of the gradient $\grad_{\bmtheta} L_{\bmx_{\leq t}}(\bmtheta)$ of the likelihood function that relies on a single stochastic sample $\bmh_{\leq t}$ for the hidden neurons. This constraint is dictated by the availability of a single compartment. The gradient used by {\VLSNN} has a generally high variance, only partially decreased by the presence of the baseline control variates in \eqref{eq:single-update}. In this section, we introduce a first learning rule that leverages multiple compartments to potentially improve the learning performance of {\VLSNN} by reducing the variance of the gradient-based updates. 


\begin{comment}
\subsection{{\MBVLSNN}: Mini-batch VLSNN}

As anticipated in Sec.~\ref{sec:intro}, in order to reduce the variance of the MC estimate in \eqref{eq:single-update}, it is possible to use a mini-batch of $K$ samples from the causally conditioned distribution \eqref{eq:causally-cond} by leveraging the availability of $K$ compartments. The resulting mini-batch variational online learning for SNNs ({\MBVLSNN}) operates as follows. 

In a $K$-compartment SNN, at each time $t=1,2,\ldots$, each compartment $k$ within the visible neurons are clamped to the respective entry in data $\bmx_{\leq t}^k$. Each hidden neuron $i \in \set{H}$ outputs $K$ binary values $\{ h_{i,t}^k \}_{k=1}^K$, with the $k$th compartment emitting a spike $h_{i,t}^k = 1$ with probability $\sigma(u_{i,t}^k)$ in \eqref{eq:spike-prob-ind}. The model parameters are updated in online manner as follows. The CP collects the binary negative cross-entropy values $\{ \bar{H}\big( x_{i,t}^k, \sigma(u_{i,t}^k) \big)\}_{k=1}^K$ of all compartments from all visible neurons $i \in \set{X}$ in order to compute the {\em per-compartment} learning signal $\ell_{\bmtheta^\text{X},t}^k$ as in \eqref{eq:single-ls}, with $u_{i,t} = u_{i,t}^k$, for the $k$th compartment. The learning signals $\{ \ell_{\bmtheta^\text{X},t}^k \}_{k=1}^K$ are then fed back from the CP to all hidden neurons $\set{H}$. The communication paths are illustrated in Fig.~\ref{fig:model-learning}.

Finally, for each neuron $i$, {\MBVLSNN} updates the local model parameters $\bmtheta_i$ by averaging the {\VLSNN} updates in \eqref{eq:single-update} over the generated $K$ samples as
\begin{subequations} \label{eq:mb-update}
\begin{align}
    &\Delta \vartheta_i =
    \begin{cases}
        \frac{1}{K} \sum_{k=1}^K \big\langle x_{i,t}^k - \sigma(u_{i,t}^k) \big\rangle_\gamma, ~\text{if}~ i \in \set{X} \\
        \frac{1}{K} \sum_{k=1}^K \big( \ell_{\bmtheta^\text{X},t}^k - b_{t}^{\vartheta_i, k} \big) \cdot \big\langle h_{i,t}^k - \sigma(u_{i,t}^k) \big\rangle_\kappa, ~\text{if}~ i \in \set{H}
    \end{cases} \label{eq:mb-update-bias} \\
    &\Delta w_{j,i} =
    \begin{cases}
        \frac{1}{K} \sum_{k=1}^K \big\langle \big( x_{i,t}^k - \sigma(u_{i,t}^k) \big) \cdot \overra{s}_{j,t-1}^{k} \big\rangle_\gamma, \\%~~\text{if}~~ i \in \set{X} \\
        \frac{1}{K} \sum_{k=1}^K \big( \ell_{\bmtheta^\text{X},t}^k - b_{t}^{w_{j,i}, k} \big) \cdot \big\langle \big( h_{i,t}^k - \sigma(u_{i,t}^k) \big) \cdot \overra{s}_{j,t-1}^{k} \big\rangle_\kappa, %~~\text{if}~~ i \in \set{H}
    \end{cases} \label{eq:mb-update-synaptic} \\
    &\Delta w_i =
    \begin{cases}
        \frac{1}{K} \sum_{k=1}^K \big\langle \big( x_{i,t}^k - \sigma(u_{i,t}^k) \big) \cdot \overla{x}_{i,t-1} \big\rangle_\gamma, \\%~~\text{if}~~ i \in \set{X} \\
        \frac{1}{K} \sum_{k=1}^K \big( \ell_{\bmtheta^\text{X},t}^k - b_{t}^{w_i, k} \big) \cdot \big\langle \big( h_{i,t}^k - \sigma(u_{i,t}^k) \big) \cdot \overla{h}_{i,t-1}^k \big\rangle_\kappa, %~~\text{if}~~ i \in \set{H}
    \end{cases} \label{eq:mb-update-feedback}
\end{align}
\end{subequations}
with time-averaging constants $\gamma, \kappa \in (0,1)$. We note that, in the update rule \eqref{eq:mb-update}, the relevance of each sample $\bmh_{\leq t}^k$ of the hidden neurons depends on the $k$th learning signal $\ell_{\bmtheta^\text{X},t}^k$. In similar manner to {\VLSNN}, for each hidden neuron $i \in \set{H}$, per-compartment baseline $\bmb_{i,t}^k$ can be optimized to minimize the variance (due to the magnitude of the per-compartment learning signal) as \cite{peters2008reinforcement}
\begin{align*}
    \bmb_{i,t}^k = \frac{\big\langle \ell_{\bmtheta^\text{X},t}^k \cdot \big(\bme_{i,t}^k\big)^2 \big\rangle_{\kappa_b} }{\big\langle \big(\bme_{i,t}^k\big)^2 \big\rangle_{\kappa_b} },
\end{align*}  
for some constant $\kappa_b \in (0,1)$, with $\bme_{i,t}^k = \langle \grad_{\bmtheta_i} \bar{H}\big( h_{i,t}^k, \sigma(u_{i,t}^k)\big) \rangle_\kappa$ being the eligibility trace at the $k$th compartment of neuron $i$ at time $t$. 

\iffalse
\begin{align*}
    \Delta \bmtheta_i = \eta \cdot 
    \begin{cases}
        \frac{1}{K} \cdot \sum_{k=1}^K \big\langle \grad_{\bmtheta_i} \bar{H}\big( x_{i,t}, \sigma(u_{i,t}^k) \big) \big\rangle, ~~\text{if}~~ i \in \set{X} \\
        \frac{1}{K} \cdot \sum_{k=1}^K \big( \ell_{\bmtheta^\text{X},t}^k - \bmb_{i,t}^k \big) \cdot \big\langle \grad_{\bmtheta_i} \bar{H} \big( h_{i,t}^k, \sigma(u_{i,t}^k) \big) \big\rangle, ~~\text{if}~~ i \in \set{H}
    \end{cases}
\end{align*}
\fi

\end{comment}

\vspace{-0.1cm}
\subsection{Communication Load}



As seen in Fig.~\ref{fig:model-learning}, {\MBVLSNN} requires computation of $K$ learning signals at CP, the resulting communication loads increase linearly to $K$. Specifically, the unicast communication load from neurons to CP is $\CNtoCP = K \CNtoCP^{(K=1)} = K |\set{X}|$ real numbers; while the broadcast communication load from CP to neurons is $\CCPtoN = K \CCPtoN^{(K=1)} = K |\set{H}|$ real numbers.


%\item A single-sample estimate of the log-likelihood of the observation heavily penalizes samples that explain the observation poorly in terms of the learning signal and thus produce low estimates of the likelihood. As a result, the variational posterior learns to cover only the high-probability areas of the true posterior, which in turn assumes a simpler shape which is easier to approximate by the variational posterior. A simple way to minimize this effect is to average over multiple samples when computing the marginal likelihood estimate. Then, one generates multiple approximate posterior samples (from the causally conditioned distribution), and their weights are averaged. The use of multiple samples gives us the additional flexibility to learn generatvie models whose posterior distributions do not fit the approximate posterior assumptions. The advantage of using a multi-sample stochastic lower bound is that increasing the number of samples is guaranteed to make the bound tighter, thus making it a better proxy for the log-likelihood. Intuitively, averaging over the $K$ samples inside the $\log$, removes the burden of every sample having to explain the observation well, which leads to the proposal distribution being considerably less concentrated than the variational posterior, which is its single-sample counterpart. Training models by optimizing a multi-sample objective can be seen as a generalization of variational training that does not explicitly represent the variational posterior.  



==> multi_learning.tex <==
\section{Multi-Sample Learning}
\label{sec:multi-learning}

\note{
\begin{enumerate}
    \item describing general idea of using multiple samples for learning: $K$ samples
    \item move the discussion on multi-sample training methods
    \item we can explain model for multi-sample training
\end{enumerate}
}


In general, probabilistic machine learning models define a parameterized joint probability $p(\bmx,\bmh)$ for observed variables $\bmx$ and latent variables $\bmh$. Recent advances in variational inference (VI) have made it possible to train such models efficiently despite the presence of possibly high-dimensional hidden variables $\bmh$. VI techniques tackle the maximization of the marginal log-likelihood of the data, namely $\log p(\bmx)$, through the maximization of the evidence lower bound (ELBO). The ELBO can be introduced via the following identity 
\begin{align}
    \log p(\bmx) = \underbrace{ \mathbb{E}_{q(\bmh)} \Big[ \log \frac{p(\bmx,\bmh)}{q(\bmh)} \Big] }_{ \text{ELBO} } + \text{KL}\big( q(\bmh) || p(\bmh|\bmx) \big),
\end{align}
where $q(\bmh)$ is an arbitrary distribution, known as variational posterior, and the term $\text{KL}\big( p||q \big) = \sum_x p(x)\log \frac{p(x)}{q(x)} \geq 0$ represents the Kullback-Leibler divergence between distributions $p$ and $q$. State-of-the-art VI methods tackle the maximization of the ELBO by iteratively optimizing over the variational posterior $q(\bmh)$ and over the model parameters defining the complete likelihood $p(\bmx,\bmh)$, through Monte Carlo (MC) sampling averages obtained by drawing samples $\bmh \sim q(\bmh)$ to evaluate expectation over $q(\bmh)$. In recent studies for ANNs, alternative approaches leveraging $K > 1$ samples from the variational posterior have been developed that optimize a more accurate lower bound on the marginal log-likelihood than the ELBO \cite{burda2015importance, tang2013sfnn, mnih2016variational, domke2018iwvi}. These lower bounds become tighter as the number $K$ of samples increases, converging to the exact value $\log p(\bmx)$ as $K \rightarrow \infty$. The resulting methods produce training algorithms based on importance weighting (IW) \cite{burda2015importance, mnih2016variational, domke2018iwvi} or generalized EM (GEM) \cite{tang2013sfnn}.  

\vspace{1cm}




References \cite{jimenez2014stochastic, brea2013matching, jang19:spm, zenke2018superspike} derived learning rules for SNNs that optimize the ELBO for given observed spiking signals $\bmx$, with a variational posterior equal to the forward distribution of the model. These techniques are based on a MC estimate of the ELBO that uses a single sample $\bmh \sim q(\bmh)$ for the hidden neurons. This allows the learning rules to be implemented in online manner by simply running the network in feedforward mode over time. 



This paper is concerned with the derivation of online local learning rules that tackle the ML problem \eqref{eq:ml}. The general form of the desired online training rule for multi-compartment SNNs follows the standard three-factor format implemented by most neuromorphic hardware \cite{fremaux2016neuromodulated, davies2018loihi}: A synaptic weight $w_{j,i}$ from pre-synaptic neuron $j$ to a post-synaptic neuron $i$ is updated as 
\begin{align} \label{eq:three-factor}
    w_{j,i} \leftarrow w_{j,i} + \eta \cdot \sum_{k=1}^K \ell^k \cdot \big\langle \text{pre}_j^k \cdot \text{post}_i^k \big\rangle,
\end{align}
where $\eta$ is the learning rate and $\langle \cdot \rangle$ denotes a time-averaging operator. The update \eqref{eq:three-factor} sums the contributions from the $K$ compartments, with each contribution depending on three different factors. The term $\text{pre}_j^k$ is a function of the filtered traces \eqref{eq:synaptic-filtered-trace} for the $(j,i)$ synapse, hence depending only on the spiking signals of the pre-synaptic neuron $j$, while the factor $\text{post}_i^k$ depends on the activity of the post-synaptic neuron $i$ processed by the $k$th compartment. Finally, $\ell^k$ is a scalar {\em learning signal} that determines the sign and magnitude of the contribution of the $k$th compartment to the learning update. The learning signal can generally be evaluated by a central processor that has access to the current outputs $(\bmx_t^k, \bmh_t^k)$ of the SNN. The learning signal $\ell^k$ may be missing in some learning rules for given subset of neurons (see Fig.~\ref{fig:model-learning} for a preview).


==> related.tex <==
\section{Related Work}
\label{sec:related}

As discussed, most of the algorithmic solutions for SNNs have been studied by assuming that each spiking neuron emits individual spikes, i.e., single-sample models \cite{jimenez2014stochastic, brea2013matching, jang19:spm, zenke2018superspike}. Several modelling and algorithmic approaches have been proposed to introduce and leverage multiple samples per neuron. A line of work including \cite{mostafa2018learning, guo2017hierarchical, jang20:vowel} considers spiking Winner-Take-All (WTA) circuits. As multiple samples per neuron are investigated here, WTA circuits maintain multiple membrane potentials per circuit. Unlike the multi-sample model, each potential is assigned to one of a group of spatially correlated spiking units in the circuit, and the potentials define a competitive process across the units through which at most one of the elements in the circuit spikes. To this end, in a WTA circuit, the weights used to compute each potential are different. This is essential in order to ensure that each element is sensitive to different spatio-temporal patterns. Therefore, increasing the number of WTA circuits entails a model with potentially more parameters, while increasing the number of samples in our model does not affect the model complexity.


\iffalse
%The spiking signals from elements in a WTA circuit are correlated and they mutually affect each other during inference. This contrasts with the parallel operation of the multiple compartments considered here. 
Other related models assume more general interconnection among compartments in order to capture the dynamic behavior of branchy dendrites \cite{ermentrout2010mathematical, drix2018sparse}. In these models, dendritic structures are treated as multiple compartments coupled with each other. In \cite{drix2018sparse}, a network of spiking neurons, each with dendritic and somatic compartments, was studied to regulate both the average firing rates and the population sparseness via separate learning rules for the compartments. Compartmentalized structures can also be effectively simulated by neuromorphic hardware with support for multi-compartment dendrites on the SpiNNaker chip \cite{furber2012spinnaker} and on Intel's Loihi \cite{davies2018loihi}.
\fi

%The reviewed existing work on multi-compartment SNN models are mostly limited to two-compartment systems or to rate-encoding solutions that apply inhibitory coupling between compartments. In contrast, in the multi-compartment model as considered in this paper, a neuron includes compartments of any size; the compartments operate independently; and the weights are shared across all compartments of a neuron. The key contribution of this work is to demonstrate that multiple compartments with shared weights can be naturally used in probabilistic models in order to obtain more effective learning rules through sampling. 


The idea of using such multi-sample objectives as a better proxy for the log-likelihood has been proposed for ANN-based variational autoencoders with continuous latent variables in \cite{burda2015importance}. This work used the reparameterization trick in order to reduce the variance of the estimator. In \cite{tang2013sfnn}, the authors proposed an importance sampling based estimator or a generalized EM bound on the log-likelihood. Focusing on the model with discrete latent variables, an unbiased gradient estimator for a multi-sample objective with per-sample learning signals was derived in \cite{mnih2016variational}.  %Reweighted wake-sleep algorithm \cite{bornschein2014reweighted} is another recognition network approach, yet training generative and recognition networks are done with different objectives \note{not clear:}.
A theoretical connection between the multi-sample objective and the log-likelihood was discussed in \cite{domke2018iwvi}. 

%The idea of IW is widely used in machine learning. For a recent application, we refer to \cite{levine2020offline} that considers the use of $K > 1$ trajectory samples from a behavior policy in area of offline reinforcement learning. In this setting, IW is leveraged to evaluate the return or the policy gradient, where the training objective is defined as the expected return under the parameterized policy.


